Deep Learning Approaches to Grasp Synthesis: A Review

Grasping is the process of picking up an object by applying forces and torques at a set of contacts. Recent advances in deep-learning methods have allowed rapid progress in robotic object grasping. In this systematic review, we surveyed the publications over the last decade, with a particular interest in grasping an object using all 6 degrees of freedom of the end-effector pose. Our review found four common methodologies for robotic grasping: sampling-based approaches, direct regression, reinforcement learning, and exemplar approaches. Additionally, we found two `supporting methods` around grasping that use deep-learning to support the grasping process, shape approximation, and affordances. We have distilled the publications found in this systematic review (85 papers) into ten key takeaways we consider crucial for future robotic grasping and manipulation research. An online version of the survey is available at https://rhys-newbury.github.io/projects/6dof/

==> definitions.tex <==
\newpage
\twocolumn

\subsection{Appendix B}


\begin{definition}[Approach vector]
\label{def:appV}
 Defines the line along which the gripper or robotic hand approach the target object \cite{morales2006}.
\end{definition}


\begin{definition}[Grasp center point]
\label{def:}
It is the point in the space aligned with the approach vector where the gripper must be positioned to start the execution of the grasp. A fixed frame of the gripper should be moved to meet the approach vector and grasp center point before the grasp is executed \cite{morales2006}.
\end{definition}

\begin{definition}[Hand orientation]
\label{def:}
Rotation of the robot hand around the approach vector when placed on the grasp center point \cite{morales2006}. 
\end{definition}


\begin{definition}[Antipodal Points]
\label{def:Antipodal_Points}
A pair of points on an objects whose normal vectors are collinear and in an opposite direction~\cite{Chen1993}. With appropriate finger contact conditions antipodal point grasps guarantee force closure. 
\end{definition}


\begin{definition}[Antipodal Grasp]
\label{def:Antipodal_Grasp}
A grasp where a two-finger gripper makes contact with the object at antipodal points~\cite{Chen1993}.
\end{definition}


\begin{definition}[Friction cone]
describes the space of normal and frictional forces that a point contact with friction can apply to the contacted surface~\cite{Nguyen1987}.
\end{definition}


\begin{definition}[Force-Closure]
\label{def:force_closure}
A force closure grasp is a set of frictional contacts which are in equilibrium for any arbitrary wrench~\cite{Nguyen1987}.
\end{definition}

\begin{definition}[Form-Closure]
An object motion is geometrically constrained in all directions by surrounding the object surface with robotic fingers~\cite{ASADA1989293}.
\end{definition}

\begin{definition}[Stable Grasp]
A grasped object at equilibrium, in which all forces and moments can be derived from a potential function V(q) is defined to be stable if $\Delta V > 0$ for every nonzero virtual displacement $\Delta q$~\cite{Howard}
\end{definition}

\begin{definition}[Grasp Wrench Space]
\label{def:Grasp_Wrench_Space}
The set of all wrenches that can be applied to the object through the grasp contacts~\cite{Borst2004}.
\end{definition}



\begin{definition}[Grasp type]
\label{def:}
A qualitative description of the grasp to be performed. This type can also define the hand preshape posture, the control strategy during the execution of the grasp, the fingers used in the execution etc. 
Feix, Iberall
\end{definition}



\begin{definition}[Hand posture]
\label{def:} The configuration of the gripper or hand fingers when the grasp is started or all the contacts are made
Needed?
\end{definition}



\begin{definition}[]
\label{def:}

\end{definition}



\begin{definition}[]
\label{def:}

\end{definition}

\begin{definition}[Power Grasp]
\label{def:PowerGrasp}
A grasp where there is multiple points of contact between the object and the fingers and palm. It maximizes the load carrying ability of a grasp and is highly stable as the enveloping nature of the grasp provides form closure~\cite{powergrasp}


\end{definition}


\begin{definition}[4DOF grasp]
\label{def:4dofgrasp}
Term used to define grasps where hand/wrist poses are generated and defined by 3D position and single orientation, commonly around the vertical axis and denoted  ${x,y,z,yaw}$.
\end{definition}


\begin{definition}[6DOF grasp]
\label{def:6dofgrasp}

Term used to define grasps where hand/wrist poses are generated and defined by the 3D position and orientation, thus 6DOF in total. 
\end{definition}


==> introOld.tex <==
Grasping and manipulation of objects using robotic arms is one of the most important tasks in robotics, with applications ranging from factory automation to service robotics. While tailored robotic grasping approaches have been developed for a range of specific scenarios, such as object handovers~\cite{yang2021reactive, Rosenberger2021}, construction~\cite{Construction2021}, mobile manipulation~\cite{mobile_manip} and agriculture~\cite{s20195670}, the most commonly investigated problem in robotic grasping is the canonical problem of picking up an item from a table with a robotic hand. 

Early approaches to robotic grasping focused on analytical methods to calculate mathematical properties describing the grasp and maximize the likelihood for success. However, these approaches tend to be slow and typically require perfect knowledge of the object model and its pose. %
% add something about the real world shortcomings? ~ Juxi
Influenced by the increased use of deep-learning in computer vision, a proliferation of works employing learning-based approaches has appeared since. The majority of recent approaches departed from contact locations as a grasp parameterization, instead trying to synthesize a grasp pose based on a camera image input. %(either RGB or RGB-D). 
Early works in deep-learning based grasp synthesis focused on `top down' or `planar grasps' with antipodal grippers. This allowed for the transfer of tools and methods from the computer vision community and also reduce the high-dimensional grasping problem to just the synthesis of four grasp pose degrees of freedom (DoF), ${x,y,z,yaw}$.
The decrease in DoF reduces the problem complexity and has enabled significant progress for vision-based grasping over the last years, it however limits their applicability. For example, if a robot needs to pick up a plate, this would not be possible by only considering a top-down grasp as the most successful approach would be to grasp the plate at the edge. 


A 6-DoF grasp pose provides the capabilities to enable robots to handle more complex grasping tasks. We differentiate between three kinds of scenes: Singulated (single object grasping), structured clutter (sparsely packed objects) and piled clutter (tightly packed objects).
We use the term 6-DoF grasping to refer to grasps with six continuous degrees of freedom. These degrees of freedom correspond to the grasp being free to translate and rotate around three perpendicular axes. However, this can be represented in various ways, commonly as a grasp point (parameterized as ${x,y,z, roll, pitch, yaw}$) or as a point and approach vector (${x,y,z,yaw, \vec{v}}$). 
Note: the gripper's DoF are not included as part of the DoF for the grasp pose, yet most approaches we reviewed did take these (at least gripper width at grasp pose) into account.


We differentiate 6-DoF grasping from Partially Discrete 6-DoF (PD6-DoF), where the latter uses all 6-DoF, however, at least one of these DoF is discrete. An example of this is~\cite{lundell2020beyond}, which uses multiple cameras placed around the scene and uses a 4-DoF approach for each camera. This allows the robot to grasp at varying pitch and roll - however, both of these angles are discrete. 



% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{images/test.JPG}
%     \caption{Top-down (or 4-DoF) grasps (red), while popular, are limited with respect to 6-DoF grasping (green) in finding more reliable and robust grasps.
%     %opens up a wide array of possible grasps even for simple shapes as boxes. This gives the robot greater ability to find stable grasps.
% }
%     \label{fig:my_label}
% \end{figure}




We herein present a systematic review of deep-learning approaches applied to 6-DoF grasping. Recent reviews in robotic grasping focus on learning-based approaches~\cite{Kleeberger2020ASO}, point-cloud based grasping~\cite{PointCloudSurvey} and manipulation~\cite{Kroemer2021ARO}. However, the recently increasing amount of deep learning approaches applied to 6-DoF grasping has not yet been systematically reviewed. 


THIS NEEDS A BIT OF GLUE

This review is based on $xxxx$ works that investigated employed deep-learning methods for grasp synthesis. We aim to find clusters of common methodologies, data sets and object-sets used. We then discuss opportunities to extend current methods.
%We limit the scope of our review to focus on approaches looking at 
Based on the papers reviewed, the following taxonomy of methods has emerged: Grasp Sampling methods, Direct Regression methods, methods incorporating Reinforcement Learning (RL) and Exemplar methods. In addition, we found deep-learning methods applied to a range of ``supporting methods'' for grasping. These methods, such as Shape Completion and Semantics/Affordances, do not directly solve the grasping problem but are increasingly employed alongside grasping approaches to increase task success.  

\begin{figure}
    \centering
    % \includegraphics[width=1\linewidth]{images/growth.png}
    \input{images/growth}
    \label{fig:my_label}
    \caption{The number of publications on IEEExplore that includes the keyword ``Grasping" in metadata and ``6DoF" in the full text. Our review is limited to deep learning within 6-DoF grasping, therefore, not all papers included in this graph are within the scope of our review.}
\end{figure}

% ***************** CAN MOVE DOWN
Authors adopt different definitions of the grasping problem. The most common definition is a pure grasp detection problem, where the input is sensor data and the output are grasp proposal(s). This commonly does not involve a temporal aspect. However, some approaches are closed-loop and involve continuous feedback. This is most commonly done in RL based approaches, which calculate an action for the robot to take, which will eventually lead to grasping. 




% IF we need space, we can always shorten/skip this
The review paper is organized as follows. The methodology used to find and extract information from relevant papers is described in Section~\ref{sec:method} and Section~\ref{sec:4dof} describes some literature on 4-DoF grasping. The following two sections focus on methods that preceded deep learning. Section~\ref{sec:Analytical_Approaches} focuses on analytical approaches and Section~\ref{sec:traditional} describes traditional machine learning methods. Section~\ref{sec:deep} presents the main findings and describes the general trends of methodologies within deep learning. The use of object sets is described and quantified in Section~\ref{sec:objects} and Section~\ref{sec:training} describes the general trends in training datasets and network backbones. Benchmarking is analyzed in Section~\ref{sec:benchmarking}, focusing on the role of simulation, grippers and metrics. The future directions are discussed in Section~\ref{sec:future}.

% Environments (why this important, where it is used)
% grasping is all over robotics
% often done on a flat surface -> this review focuses on table top settings
%  grasping can either be done just to pick it up or can be done in terms of semantics (how to grasp classes of objects)

% What is 6Dof Grasping? 
% % Define Key Terms
% % Clutter, DoF
% We define 4-DoF grasping to use 4-DoF in a continous manner. These 4 degrees of freedom are (x,y,z, yaw). 

% We define 6-DoF grasping to be using a 6-DoF in a continuous manner. This means, that the graspoing pose should be able to have continous movement in all 6 degrees of freedom (x,y,z, roll, pitch, yaw)

% We differentiation this from Partially Discrete 6-DoF (PoF) systems. These system have at least one of the degrees freedom is discritzed. 

% What is the structure...


% discuss evolution of DOF (6 -> 4 -> 6?)


==> table.tex <==
% \begin{table*}
    % \centering
% \begin{tabular} 
\clearpage

\onecolumn

% \juxitodo{i liked the first author name in the column}

\begin{longtable}{| c ? c ? c ? c | c | c | c ? c ? c | c | c | c | c | c | c | c |}
\hline


\rowcolor[HTML]{D0CECE}
Year & Paper & Method & Train & Test & Gripper & Clutter & PD & SR & Cov & Com & GP & CT & IOU & P & Impact \\ \hline
\rowcolor[HTML]{ffffff}
2019 & Mousavian~\cite{mousavian20196} & Sampling & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 2.68\\ \hline
\rowcolor[HTML]{f0f0f5}
2017 & ten Pas~\cite{ten2017grasp} & Sampling & Sim & Real & Two-Finger & Dense &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 2.22\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Fang~\cite{fang2020graspnet} & Direct Regression & Hybrid & Real & Two-Finger & Sparse &  & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 2.13\\ \hline
\rowcolor[HTML]{f0f0f5}
2016 & Gualtieri~\cite{gualtieri2017high} & Sampling & Sim & Real & Two-Finger & Dense &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 2.06\\ \hline
\rowcolor[HTML]{ffffff}
2017 & Varley~\cite{varley2017shape} & Shape Completion & Sim & Real & High-DoF & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.91\\ \hline
\rowcolor[HTML]{f0f0f5}
2020 & Murali~\cite{murali20206} & Sampling & Sim & Real & Two-Finger & Sparse &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.68\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Wu~\cite{wu2020grasp} & Direct Regression & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.64\\ \hline
\rowcolor[HTML]{f0f0f5}
2018 & Choi~\cite{choi2018soft} & Direct Regression & Real & Real & Soft Hand & Singulated & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 1.59\\ \hline
\rowcolor[HTML]{ffffff}
2015 & Varley~\cite{varley2015generating} & Sampling & Sim & Real & High-DoF  & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.53\\ \hline
\rowcolor[HTML]{f0f0f5}
2019 & Liang~\cite{Liang_2019} & Sampling & Sim & Sim & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.52\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Van der Merwe~\cite{vandermerwe2020learning} & Shape Completion & Sim & Real & High-DoF & Singulated &  & \ForestGreencheck &  &  &  &  & \ForestGreencheck &  & 1.51\\ \hline
\rowcolor[HTML]{f0f0f5}
2020 & Ni~\cite{ni2020pointnet} & Direct Regression & Sim & Real & Two-Finger & Dense &  & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  & 1.41\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Lundell~\cite{lundell2020beyond} & Shape Completion & Sim & Real & Two-Finger & Dense & \ForestGreencheck & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  & 1.41\\ \hline
\rowcolor[HTML]{f0f0f5}
2020 & Song~\cite{song2020grasping} & LfD, RL & Real & Real & Two-Finger & Dense &  & \ForestGreencheck &  &  &  &  &  &  & 1.38\\ \hline
\rowcolor[HTML]{ffffff}
2021 & Zhao~\cite{zhao2020regnet} & Direct Regression & Sim & Real & Two-Finger & Dense &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 1.38\\ \hline
\rowcolor[HTML]{f0f0f5}
2019 & Lundell~\cite{Lundell2019} & Shape Completion & Sim & Real & High-DoF & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.36\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Lou~\cite{lou2020learning} & Sampling & Sim & Real & Two-Finger & Dense &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 1.36\\ \hline
\rowcolor[HTML]{f0f0f5}
2020 & Qin~\cite{qin2020s4g} & Direct Regression & Sim & Real & Two-Finger & Dense &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 1.34\\ \hline
\rowcolor[HTML]{ffffff}
2021 & Gou~\cite{gou2021rgb} & Sampling & Hybrid & Real & Two-Finger & Sparse & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 1.33\\ \hline
\rowcolor[HTML]{f0f0f5}
2021 & Lundell~\cite{lundell2021multifingan} & Shape Completion & Sim & Real & High-DoF & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.33\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Choi~\cite{choi2020hierarchical} & Direct Regression & Sim & Real & Two-Finger & \specialcell{Sparse\\Dense} &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.30\\ \hline
\rowcolor[HTML]{f0f0f5}
2021 & Sundermeyer~\cite{sundermeyer2021contactgraspnet} & Direct Regression & Sim & Real & Two-Finger & Sparse &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.30\\ \hline
\rowcolor[HTML]{ffffff}
2021 & Lou~\cite{lou2021collisionaware} & Sampling & Sim & Real & Two-Finger & Sparse &  & \ForestGreencheck &  &  &  &  &  &  & 1.30\\ \hline
\rowcolor[HTML]{f0f0f5}
2021 & Zhu~\cite{zhu20216dof} & Direct Regression & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.30\\ \hline
\rowcolor[HTML]{ffffff}
2021 & Berscheid~\cite{berscheid2021robot} & RL & Real & Real & Two-Finger & Dense &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.30\\ \hline
\rowcolor[HTML]{f0f0f5}
2019 & Wu~\cite{wu2019pixel} & RL & Sim & Real & High-DoF & Dense &  & \ForestGreencheck &  &  &  &  &  &  & 1.28\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Lu~\cite{lu2020multi} & Active Learning & Sim & Real & High-DoF  & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.27\\ \hline
\rowcolor[HTML]{f0f0f5}
2018 & Gualtieri~\cite{gualtieri2018learning} & RL & Sim & Real & Two-Finger & Sparse &  & \ForestGreencheck &  &  &  &  &  &  & 1.26\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Wu~\cite{wu2020generative} & RL & Sim & Real & \specialcell{Two-Finger\\High-DoF} & \specialcell{Singulated\\Dense} &  & \ForestGreencheck &  &  &  &  &  &  & 1.23\\ \hline
\rowcolor[HTML]{f0f0f5}
2021 & Gualtieri~\cite{gualtieri2021robotic} & Shape Completion & Sim & Real & Two-Finger & Sparse &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 1.21\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Kiatos~\cite{Kiatos2020} & Shape Completion & Sim & Real & High-DoF & Sparse &  & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  & 1.20\\ \hline
\rowcolor[HTML]{f0f0f5}
2020 & Breyer~\cite{breyer2021volumetric} & Direct Regression & Sim & Real & Two-Finger & Dense &  & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  & 1.14\\ \hline
\rowcolor[HTML]{ffffff}
2019 & Liu~\cite{liu2019generating} & Direct Regression & Sim & Real & High-DoF & Singulated &  &  &  &  &  &  &  &  & 1.13\\ \hline
\rowcolor[HTML]{f0f0f5}
2019 & Ottenhaus~\cite{ottenhaus2019visuo} & Shape Completion & Sim & Real & High-DoF & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.13\\ \hline
\rowcolor[HTML]{ffffff}
2019 & Gao~\cite{gao2019kpamsc} & Affordances & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.12\\ \hline
\rowcolor[HTML]{f0f0f5}
2020 & Liu~\cite{liu2020deep} & Direct Regression & Sim & Real & High-DoF  & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.12\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Lu~\cite{lu2020multifingered} & Direct Regression & Sim & Real & High-DoF & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.10\\ \hline
\rowcolor[HTML]{f0f0f5}
2019 & Yan~\cite{yan2019dataefficient} & Sampling & Sim & Real & Two-Finger & Sparse &  & \ForestGreencheck &  &  &  &  & \ForestGreencheck &  & 1.09\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Ni~\cite{ni2021learning} & Direct Regression & Sim & Real & Two-Finger & Sparse &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 1.08\\ \hline
\rowcolor[HTML]{f0f0f5}
2021 & Wang~\cite{wang2021goalauxiliary} & RL, LfD & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.03\\ \hline
\rowcolor[HTML]{ffffff}
2021 & Wang~\cite{Wang2021} & Sampling & Hybrid & Real & Two-Finger & Sparse &  & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  & 1.02\\ \hline
\rowcolor[HTML]{f0f0f5}
2020 & Schaub~\cite{Schaub2020} & Sampling & Sim & Real & Two-Finger & Singulated & \ForestGreencheck &  &  &  &  &  &  &  & 1.02\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Lu~\cite{lu2019planning} & Sampling & Sim & Real & \specialcell{High-DoF\\Two-Finger} & Singulated &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 1.00\\ \hline
\rowcolor[HTML]{f0f0f5}
2021 & Jiang~\cite{jiang2021synergies} & Shape Completion & Sim & Real & Two-Finger & Dense &  & \ForestGreencheck & \ForestGreencheck &  &  &  & \ForestGreencheck &  & 1.00\\ \hline
\rowcolor[HTML]{ffffff}
2021 & Lundell~\cite{lundell2021ddgc} & Shape Completion & Sim & Real & Two-Finger & Sparse &  &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  & 1.00\\ \hline
\rowcolor[HTML]{f0f0f5}
2021 & Munoz~\cite{munoz2021grasping} & Direct Regression & Sim & Real & Two-Finger & Singulated & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 1.00\\ \hline
\rowcolor[HTML]{ffffff}
2021 & Peng~\cite{peng2021selfsupervised} & Sampling & Sim & Real & Two-Finger & Sparse &  & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  & 1.00\\ \hline
\rowcolor[HTML]{f0f0f5}
2021 & Kasaei~\cite{kasaei2021mvgrasp} & Direct Regression & Real & Real & Two-Finger & \specialcell{Singulated\\Dense} & \ForestGreencheck & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck & \ForestGreencheck &  & 1.00\\ \hline
\rowcolor[HTML]{ffffff}
2018 & Schmidt~\cite{Schmidt2018} & Direct Regression & Sim & Real* & High-DoF & Singulated &  &  &  &  &  &  &  &  & 0.80\\ \hline
\rowcolor[HTML]{f0f0f5}
2018 & Yan~\cite{yan2018learning} & LfD & Sim & Sim & Two-Finger & Singulated &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 0.63\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Murali~\cite{murali2020same} & Sampling & Sim & Real* & Two-Finger & Singulated &  &  &  &  &  &  &  & \ForestGreencheck & 0.62\\ \hline
\rowcolor[HTML]{f0f0f5}
2021 & Tang~\cite{Tang2021LearningCP} & RL & Sim & Real* & Two-Finger & Dense &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 0.50\\ \hline
\rowcolor[HTML]{ffffff}
2019 & Tian~\cite{tian2019transferring} & Affordances, Other & Sim & Sim & High-DoF & Singulated &  &  &  &  &  & \ForestGreencheck &  &  & 0.36\\ \hline
\rowcolor[HTML]{f0f0f5}
2020 & Patten~\cite{patten2020dgcm} & Other & Sim &  & Two-Finger & Singulated &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 0.15\\ \hline 
\rowcolor[HTML]{ffffff}
2020 & Li~\cite{li2020learning} & Affordances & Sim & Sim & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  &  & \ForestGreencheck &  & 0.13\\ \hline
\rowcolor[HTML]{f0f0f5}
2017 & Zhou~\cite{zhou20176dof} & Sampling & Sim & Sim & High-DoF & Singulated &  &  &  &  & \ForestGreencheck &  &  &  & 0.10\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Jeng~\cite{jeng2020gdn} & Direct Regression & Sim & Sim & Two-Finger & \specialcell{Singulated\\Sparse} &  & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  & \ForestGreencheck & 0.09\\ \hline
\rowcolor[HTML]{f0f0f5}
2018 & Torii~\cite{Torii2018} & Shape Completion & Sim & Sim & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.09\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Mandikal~\cite{mandikal2020graff} & Affordances, RL & Sim & Sim & High-DoF  & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.05\\ \hline
\rowcolor[HTML]{f0f0f5}
2020 & Yang~\cite{yang2020robotic} & \specialcell{Direct Regression\\Shape Completion} & Sim & Sim & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.01\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Riedlinger~\cite{Riedlinger2020} & Sampling & Sim & Sim & Two-Finger & Singulated &  &  &  &  &  &  &  & \ForestGreencheck & 0.01\\ \hline
\rowcolor[HTML]{f0f0f5}
2021 & Kawakami~\cite{kawakami2021learning} & RL, LfD & Sim & Sim & Two-Finger & Singulated &  &  &  &  &  &  &  &  & 0.00\\ \hline
\rowcolor[HTML]{ffffff}
2020 & Avigal~\cite{avigal20206dof} & Shape Completion & Sim & Sim & Two-Finger & Singulated &  &  &  &  &  &  &  &  & 0.00\\ \hline
\rowcolor[HTML]{ffffff}
2019 & Gonçalves~\cite{Goncalves2019} & & & & & & & & & & & & & & \\ \hline
2020 & Wang~\cite{Wang2020} & & & & & & & & & & & & & & \\ \hline
2021 & Corten~\cite{Cortes2021} & & & & & & & & & & & & & & \\ \hline
2021 & Wang~\cite{Wang2021} & & & & & & & & & & & & & & \\ \hline
2021 & Wen~\cite{wencatgrasp} & & & & & & & & & & & & & & \\ \hline
2021 & Li~\cite{Li2021} & & & & & & & & & & & & & & \\ \hline
2020 & Riccardo~\cite{Riccardo2020} & & & & & & & & & & & & & & \\ \hline
2021 & Schuab~\cite{Schuab2021} & & & & & & & & & & & & & & \\ \hline
2021 & Ren~\cite{Ren2021} & & & & & & & & & & & & & & \\ \hline
2021 & Chavan-Dafle~\cite{chavandafle2021object} & & & & & & & & & & & & & & \\ \hline
2021 & Li~\cite{li2021simultaneous} & & & & & & & & & & & & & & \\ \hline
2021 & Corsaro~\cite{corsaro2021learning} & & & & & & & & & & & & & & \\ \hline
2021 & Wei~\cite{wei2021gpr} & & & & & & & & & & & & & & \\ \hline
2019 & Aktas~\cite{aktas2019deep} & & & & & & & & & & & & & & \\ \hline
2020 & Chen~\cite{chen2020transferable} & & & & & & & & & & & & & & \\ \hline
2017 & Veres~\cite{Veres2017} & & & & & & & & & & & & & & \\ \hline
2019 & Ardon~\cite{Ardon2019} & & & & & & & & & & & & & & \\ \hline
2017 & Nguyen~\cite{Nguyen2017} & & & & & & & & & & & & & & \\ \hline
2016 & Nguyen~\cite{nguyen2016detecting} & & & & & & & & & & & & & & \\ \hline
2020 & Kokic~\cite{Kokic2020} & & & & & & & & & & & & & & \\ \hline

% \end{tabular}
\caption{Properties of the papers in this systematic review.
"PD" indicates whether the grasping approach was partial 6-DoF, refer to Sec. TODO.
"SR", "Cov", "Com", "CT", "IOU" and "P" refer to Success Rate, Coverage Rate, Completion Rate, Computation Time, Intersection of Union and Precision which were the metrics used in the paper, refer to Sec.~\ref{sec:metrics}.
"Impact" is the impact described in Section~\ref{quality_score}.\\}
\label{big_table}
\end{longtable}
% \end{landscape}



==> table_update2.tex <==
\clearpage

\onecolumn
\section{Appendices}
\subsection{Appendix A}
% \tiny
\footnotesize

\begin{longtable}{| c ? c ? c ? c | c | c | c | c | c | c ? c ? c | c | c | c | c | c | c | c |}
\hline
\rowcolor[HTML]{D0CECE}
Year & Paper & Method & SC & S/A & LfD & Train & Test & Gripper & Clutter & PD & SR & Cov & Com & GP & CT & IOU & P & Impact \\ \hline
2019 & Mousavian~\cite{mousavian20196} & Sampling &  &  &  & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 2.36\\ \hline
2020 & Fang~\cite{fang2020graspnet} & Direct Regression &  &  &  & Hybrid & Real & Two-Finger & Structured &  & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 2.35\\ \hline
2017 & ten Pas~\cite{ten2017grasp} & Sampling &  &  &  & Sim & Real & Two-Finger & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 2.22\\ \hline
2016 & Gualtieri~\cite{gualtieri2017high} & Sampling &  &  &  & Sim & Real & Two-Finger & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.95\\ \hline
2020 & Murali~\cite{murali20206} & Sampling &  &  &  & Sim & Real & Two-Finger & Structured &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 1.94\\ \hline
2017 & Varley~\cite{varley2017shape} & Analytical & \ForestGreencheck &  &  & Sim & Real & Three-Finger & \specialcell{Singulated\\Structured} &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.88\\ \hline
2020 & Wu~\cite{wu2020grasp} & Direct Regression &  &  &  & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 1.69\\ \hline
2016 & Nguyen~\cite{nguyen2016detecting} & Analytical &  & \ForestGreencheck &  & Real & Real & Multi-Fingered & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.64\\ \hline
2018 & Choi~\cite{choi2018soft} & Direct Regression &  &  &  & Real & Real & Soft Hand & Singulated & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 1.60\\ \hline
2021 & Sundermeyer~\cite{sundermeyer2021contactgraspnet} & Direct Regression &  &  &  & Sim & Real & Two-Finger & Structured &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 1.60\\ \hline
2020 & Song~\cite{song2020grasping} & RL &  &  & \ForestGreencheck & Real & Real & Two-Finger & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 1.58\\ \hline
2020 & Merwe~\cite{vandermerwe2020learning} & Sampling &  &  &  & Sim & Real & Multi-Fingered & Singulated &  & \ForestGreencheck &  &  &  &  & \ForestGreencheck &  & 1.57\\ \hline
2019 & Lu~\cite{lu2019planning} & Sampling &  &  &  & Sim & Real & \specialcell{Two-Finger\\Multi-Fingered} & Singulated &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 1.54\\ \hline
2017 & Nguyen~\cite{Nguyen2017} & Analytical &  &  &  & Real* & Real & Multi-Fingered & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 1.54\\ \hline
2015 & Varley~\cite{varley2015generating} & Sampling &  &  &  & Sim & Real & Three-Finger & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.49\\ \hline
2020 & Qin~\cite{qin2020s4g} & Direct Regression &  &  &  & Sim & Real & Two-Finger & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.45\\ \hline
2020 & Shao~\cite{shao2020unigrasp} & Direct Regression &  &  &  & Sim & Real & Multi-Fingered & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.45\\ \hline
2019 & Gao~\cite{gao2019kpamsc} & Analytical & \ForestGreencheck & \ForestGreencheck &  & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.43\\ \hline
2021 & Zhao~\cite{zhao2020regnet} & Direct Regression &  &  &  & Sim & Real & Two-Finger & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.42\\ \hline
2020 & Lundell~\cite{lundell2020beyond} & Sampling & \ForestGreencheck &  &  & Sim & Real & Two-Finger & Piled & \ForestGreencheck & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.41\\ \hline
2020 & Kokic~\cite{Kokic2020} & Direct Regression &  & \ForestGreencheck &  & Sim & Real & Two-Finger & Singulated &  &  &  &  &  &  &  & \ForestGreencheck & 1.41\\ \hline
2021 & Wang~\cite{Wang_2021_ICCV} & Direct Regression &  &  &  & Hybrid & Real & Two-Finger & Piled &  & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 1.40\\ \hline
2020 & Lou~\cite{lou2020learning} & Sampling &  &  &  & Sim & Real & Two-Finger & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.38\\ \hline
2019 & Lundell~\cite{Lundell2019} & Analytical & \ForestGreencheck &  &  & Sim & Real & Three-Finger & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.37\\ \hline
2021 & Gou~\cite{gou2021rgb} & Direct Regression &  &  &  & Hybrid & Real & Two-Finger & Structured & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 1.36\\ \hline
2021 & Lundell~\cite{lundell2021multifingan} & Sampling & \ForestGreencheck &  &  & Sim & Real & Three-Finger & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.36\\ \hline
2021 & Lou~\cite{lou2021collisionaware} & Sampling &  &  &  & Sim & Real & Two-Finger & Structured &  & \ForestGreencheck &  &  &  &  &  &  & 1.34\\ \hline
2020 & Chen~\cite{chen2020transferable} & RL &  &  & \ForestGreencheck & Sim & Real & Two-Finger & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 1.34\\ \hline
2020 & Choi~\cite{choi2020hierarchical} & Direct Regression &  &  &  & Sim & Real & Two-Finger & \specialcell{Structured\\Piled} &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.32\\ \hline
2021 & Zhu~\cite{zhu20216dof} & Direct Regression &  &  &  & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.32\\ \hline
2021 & Berscheid~\cite{berscheid2021robot} & RL &  &  &  & Real & Real & Two-Finger & Piled &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.32\\ \hline
2021 & Wei~\cite{wei2021gpr} & Direct Regression &  &  &  & Sim & Real & Two-Finger & Piled &  & \ForestGreencheck & \ForestGreencheck & \ForestGreencheck &  &  &  &  & 1.32\\ \hline
2019 & Liu~\cite{liu2019generating} & Direct Regression &  &  &  & Sim & Real & Multi-Fingered & Singulated &  &  &  &  &  &  &  &  & 1.31\\ \hline
2020 & Ni~\cite{ni2020pointnet} & Direct Regression &  &  &  & Sim & Real & Two-Finger & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.30\\ \hline
2019 & Wu~\cite{wu2019pixel} & RL &  &  &  & Sim & Real & Three-Finger & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 1.30\\ \hline
2020 & Lu~\cite{lu2020multi} & Active Learning &  &  &  & Sim & Real & Multi-Fingered  & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.28\\ \hline
2020 & Wu~\cite{wu2020generative} & RL &  &  &  & Sim & Real & \specialcell{Two-Finger\\Multi-Fingered} & \specialcell{Singulated\\Piled} &  & \ForestGreencheck &  &  &  &  &  &  & 1.28\\ \hline
2019 & Ardon~\cite{Ardon2019} & Direct Regression &  & \ForestGreencheck &  & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.28\\ \hline
2021 & Gualtieri~\cite{gualtieri2021robotic} & Analytical & \ForestGreencheck &  &  & Sim & Real & Two-Finger & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.26\\ \hline
2021 & Lundell~\cite{lundell2021ddgc} & Sampling & \ForestGreencheck &  &  & Sim & Real & Three-Finger & Structured &  &  &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.26\\ \hline
2018 & Gualtieri~\cite{gualtieri2018learning} & RL &  &  &  & Sim & Real & Two-Finger & Structured &  & \ForestGreencheck &  &  &  &  &  &  & 1.26\\ \hline
2020 & Kiatos~\cite{Kiatos2020} & Analytical & \ForestGreencheck &  &  & Sim & Real & Three-Finger & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.24\\ \hline
2020 & Breyer~\cite{breyer2021volumetric} & Direct Regression &  &  &  & Sim & Real & Two-Finger & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.23\\ \hline
2016 & Mahler~\cite{Dexnet1} & \specialcell{Sampling\\Exemplar} & \ForestGreencheck & \ForestGreencheck &  & Sim & Sim & Two-Finger & Singulated &  &  &  &  &  &  &  &  & 1.22\\ \hline
2021 & Li~\cite{li2021simultaneous} & Direct Regression &  & \ForestGreencheck &  & Sim & Real & Two-Finger & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  & \ForestGreencheck & 1.19\\ \hline
2021 & Corsaro~\cite{corsaro2021learning} & Sampling &  &  &  & Sim & Real & Multi-Fingered & Structured &  & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 1.19\\ \hline
2020 & Lu~\cite{lu2020multifingered} & Direct Regression &  &  &  & Sim & Real & Multi-Fingered & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.18\\ \hline
2020 & Patten~\cite{patten2020dgcm} & Other &  &  &  & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 1.18\\ \hline
2020 & Liu~\cite{liu2020deep} & Direct Regression &  &  &  & Sim & Real & Multi-Fingered  &  &  & \ForestGreencheck &  &  &  &  &  &  & 1.14\\ \hline
2019 & Ottenhaus~\cite{ottenhaus2019visuo} & Sampling & \ForestGreencheck &  &  & Sim & Real & Multi-Fingered & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.13\\ \hline
2021 & Peng~\cite{peng2021selfsupervised} & Sampling &  &  &  & Sim & Real & Two-Finger & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.10\\ \hline
2021 & Jiang~\cite{jiang2021synergies} & Sampling & \ForestGreencheck &  &  & Sim & Real & Two-Finger & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  & \ForestGreencheck &  & 1.08\\ \hline
2020 & Ni~\cite{ni2021learning} & Direct Regression &  &  &  & Sim & Real & Two-Finger & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.07\\ \hline
2019 & Gonçalves~\cite{Goncalves2019} & Sampling &  &  &  & Sim & Real & Three-Finger & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.07\\ \hline
2021 & Corten~\cite{Cortes2021} & RL &  &  & \ForestGreencheck & Real & Real & Multi-Fingered & Structured &  & \ForestGreencheck &  &  &  &  &  &  & 1.06\\ \hline
2021 & Kasaei~\cite{kasaei2021mvgrasp} & Direct Regression &  &  &  & Real & Real & Two-Finger & \specialcell{Singulated\\Piled} & \ForestGreencheck & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck & \ForestGreencheck &  & 1.04\\ \hline
2019 & Aktas~\cite{aktas2019deep} & Sampling &  &  & \ForestGreencheck & Sim & Real & Multi-Fingered & Singulated &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 1.03\\ \hline
2020 & Schaub~\cite{Schaub2020} & Sampling &  &  &  & Real & Real & Two-Finger & Singulated & \ForestGreencheck &  &  &  &  &  &  &  & 1.03\\ \hline
2021 & Wang~\cite{Wang2021} & Sampling &  &  &  & Hybrid & Real & Two-Finger & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.02\\ \hline
2021 & Wang~\cite{wang2021goalauxiliary} & RL &  &  & \ForestGreencheck & Sim & Real & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.02\\ \hline
2020 & Wang~\cite{Wang2020} & Direct Regression &  &  &  & Sim & Real & \specialcell{Two-Finger\\Multi-Fingered} & \specialcell{Structured\\Piled} &  & \ForestGreencheck &  &  &  &  &  &  & 1.01\\ \hline
2021 & Ren~\cite{Ren2021} & Sampling &  &  &  & Sim & Real & Two-Finger & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.01\\ \hline
2018 & Schmidt~\cite{Schmidt2018} & Direct Regression &  &  &  & Sim & Demo & Multi-Fingered & Singulated &  &  &  &  &  &  &  &  & 1.01\\ \hline
2021 & Li~\cite{Li2021} & Direct Regression &  &  &  & Sim & Real & Multi-Fingered & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.01\\ \hline
2019 & Liang~\cite{Liang_2019} & Sampling &  &  &  & Sim & Sim & Three-Finger & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 1.00\\ \hline
2021 & Wen~\cite{wencatgrasp} & Sampling &  & \ForestGreencheck &  & Sim & Real & Two-Finger & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 1.00\\ \hline
2021 & Schuab~\cite{Schuab2021} & Sampling & \ForestGreencheck &  &  &  & Real & Two-Finger & Singulated & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  &  & 1.00\\ \hline
2021 & Chavan-Dafle~\cite{chavandafle2021object} & Analytical & \ForestGreencheck &  &  & Sim & Real & Two-Finger & Structured &  & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 1.00\\ \hline
2015 & Kappler~\cite{bohg2015dataset} & Sampling &  &  &  & Sim & Sim & Three-Finger & Sigulated &  &  &  &  &  &  &  &  & 0.91\\ \hline
2021 & Tang~\cite{Tang2021LearningCP} & RL &  &  &  & Sim & Demo & Two-Finger & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 0.82\\ \hline
2020 & Murali~\cite{murali2020same} & Sampling &  &  &  & Sim & Demo & Two-Finger & Singulated &  &  &  &  &  &  &  & \ForestGreencheck & 0.64\\ \hline
2018 & Yan~\cite{yan2018learning} & Sampling & \ForestGreencheck &  & \ForestGreencheck & Sim & Sim & Two-Finger & Singulated &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 0.59\\ \hline
2019 & Merzic~\cite{2019_ICRA_mbkrb} & RL &  &  &  & Sim & Sim & Three-Finger &  &  & \ForestGreencheck &  &  &  &  &  &  & 0.50\\ \hline
2021 & Munoz~\cite{munoz2021grasping} & Direct Regression &  &  &  & Sim & Demo & Two-Finger & Singulated & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 0.50\\ \hline
2020 & Mandikal~\cite{mandikal2020graff} & RL &  & \ForestGreencheck &  & Sim & Sim & Multi-Fingered  & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.37\\ \hline
2020 & Yang~\cite{yang2020robotic} & Direct Regression & \ForestGreencheck &  &  & Sim & Sim & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.33\\ \hline
2017 & Veres~\cite{Veres2017} & Sampling &  &  &  & Sim & Sim & Three-Finger & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.33\\ \hline
2020 & Riccardo~\cite{Riccardo2020} & GPD &  & \ForestGreencheck &  & - & - &  &  &  &  &  &  &  &  &  &  & 0.26\\ \hline
2020 & Li~\cite{li2020learning} & Analytical &  & \ForestGreencheck &  & Sim & Sim & Two-Finger & Singulated &  & \ForestGreencheck &  &  &  &  & \ForestGreencheck &  & 0.13\\ \hline
2020 & Jeng~\cite{jeng2020gdn} & Direct Regression &  &  &  & Sim & Sim & Two-Finger & \specialcell{Singulated\\Structured} &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck & 0.09\\ \hline
2018 & Torii~\cite{Torii2018} & Analytical & \ForestGreencheck &  &  & Sim & Sim & Three-Finger & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.09\\ \hline
2017 & Zhou~\cite{zhou20176dof} & Sampling &  &  &  & Sim & Sim & Three-Finger & Singulated &  &  &  &  & \ForestGreencheck &  &  &  & 0.08\\ \hline
2020 & Riedlinger~\cite{Riedlinger2020} & Sampling &  &  &  & Sim & Sim & Two-Finger & Singulated &  &  &  &  &  &  &  & \ForestGreencheck & 0.03\\ \hline
2020 & Avigal~\cite{avigal20206dof} & Shape Completion & \ForestGreencheck &  &  & Sim & Sim & Two-Finger & Singulated & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  &  & 0.02\\ \hline
2021 & Kawakami~\cite{kawakami2021learning} & RL &  &  & \ForestGreencheck & Sim & Sim & Two-Finger & Singulated &  &  &  &  &  &  &  &  & 0.00\\ \hline

\caption{The papers included in this systematic review ordered by our impact score (Section~\ref{sec:method}).
The various properties are presented for easy comparison.
``PD" indicates whether the grasping approach was partial 6-DoF. ``MF" represents a Multi-Fingered hand, while ``2F", ``3F" refer to Two-Finger and Three Finger respectively.
``SC" referes to if the appraoch used Shape Completion. ``SA" refers to Semantics/Affordances.
``SR", ``Cov", ``Com", ``CT", ``IOU" and ``P" refer to Success Rate, Coverage Rate, Completion Rate, Computation Time, Intersection of Union and Precision which were the metrics used in the paper, refer to Sec.~\ref{sec:metrics}.
``Impact" is the impact described in Section~\ref{quality_score}. *This data contains no grasping information.\\}
\label{big_table}
\end{longtable}

==> table_updated.tex <==
\clearpage

\onecolumn
\section{Appendices}
\subsection{Appendix A}
\begin{longtable}{| c ? c ? c ? c | c | c | c | c | c | c ? c ? c | c | c | c | c | c | c | c |}
\hline
\rowcolor[HTML]{D0CECE}
Year & Paper & Method & SC & S/A & LfD & Train & Test & Gripper & Clutter & PD & SR & Cov & Com & GP & CT & IOU & P & Impact \\ \hline
2019 & \cite{mousavian20196} & Sampling &  &  &  & Sim & Real & 2F & Singulated &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 2.36\\ \hline
2020 & \cite{fang2020graspnet} & Direct Regression &  &  &  & Hybrid & Real & 2F & Structured &  & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 2.35\\ \hline
2017 & \cite{ten2017grasp} & Sampling &  &  &  & Sim & Real & 2F & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 2.22\\ \hline
2019 & \cite{Liang_2019} & Sampling &  &  &  & Sim & Sim & 2F & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 2.00\\ \hline
2016 & \cite{gualtieri2017high} & Sampling &  &  &  & Sim & Real & 2F & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.95\\ \hline
2020 & \cite{murali20206} & Sampling &  &  &  & Sim & Real & 2F & Structured &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 1.94\\ \hline
2017 & \cite{varley2017shape} & Analytical & \ForestGreencheck &  &  & Sim & Real & MF & \specialcell{Singulated\\Structured} &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.88\\ \hline
2020 & \cite{wu2020grasp} & Sampling &  &  &  & Sim & Real & 2F & Singulated &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 1.69\\ \hline
2018 & \cite{choi2018soft} & Direct Regression &  &  &  & Real & Real & Soft & Singulated & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 1.60\\ \hline
2021 & \cite{sundermeyer2021contactgraspnet} & Direct Regression &  &  &  & Sim & Real & 2F & Structured &  & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & 1.60\\ \hline
2020 & \cite{song2020grasping} & RL &  &  & \ForestGreencheck & Real & Real & 2F & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 1.58\\ \hline
2020 & \cite{vandermerwe2020learning} & Sampling &  &  &  & Sim & Real & MF & Singulated &  & \ForestGreencheck &  &  &  &  & \ForestGreencheck &  & 1.57\\ \hline
2019 & \cite{lu2019planning} & Sampling &  &  &  & Sim & Real & MF/2F & Singulated &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 1.54\\ \hline
2015 & \cite{varley2015generating} & Sampling &  &  &  & Sim & Real & MF & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.49\\ \hline
2020 & \cite{qin2020s4g} & Direct Regression &  &  &  & Sim & Real & 2F & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.45\\ \hline
2019 & \cite{gao2019kpamsc} & Analytical & \ForestGreencheck & \ForestGreencheck &  & Sim & Real & 2F & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.43\\ \hline
2021 & \cite{zhao2020regnet} & Direct Regression &  &  &  & Sim & Real & 2F & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.42\\ \hline
2020 & \cite{lundell2020beyond} & Sampling & \ForestGreencheck &  &  & Sim & Real & 2F & Piled & \ForestGreencheck & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.41\\ \hline
2020 & \cite{lou2020learning} & Sampling &  &  &  & Sim & Real & 2F & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.38\\ \hline
2019 & \cite{Lundell2019} & Analytical & \ForestGreencheck &  &  & Sim & Real & MF & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.37\\ \hline
2021 & \cite{gou2021rgb} & Direct Regression &  &  &  & Hybrid & Real & 2F & Structured & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 1.36\\ \hline
2021 & \cite{lundell2021multifingan} & Sampling & \ForestGreencheck &  &  & Sim & Real & MF & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.36\\ \hline
2021 & \cite{lou2021collisionaware} & Sampling &  &  &  & Sim & Real & 2F & Structured &  & \ForestGreencheck &  &  &  &  &  &  & 1.34\\ \hline
2020 & \cite{choi2020hierarchical} & Direct Regression &  &  &  & Sim & Real & 2F & \specialcell{Structured\\Piled} &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.32\\ \hline
2021 & \cite{zhu20216dof} & Direct Regression &  &  &  & Sim & Real & 2F & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.32\\ \hline
2021 & \cite{berscheid2021robot} & RL &  &  &  & Real & Real & 2F & Piled &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.32\\ \hline
2019 & \cite{liu2019generating} & Direct Regression &  &  &  & Sim & Real & MF & Singulated &  &  &  &  &  &  &  &  & 1.31\\ \hline
2020 & \cite{ni2020pointnet} & Direct Regression &  &  &  & Sim & Real & 2F & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.30\\ \hline
2019 & \cite{wu2019pixel} & RL &  &  &  & Sim & Real & MF & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 1.30\\ \hline
2020 & \cite{lu2020multi} & Active Learning &  &  &  & Sim & Real & MF & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.28\\ \hline
2020 & \cite{wu2020generative} & RL &  &  &  & Sim & Real & \specialcell{MF/2F} & \specialcell{Singulated\\Piled} &  & \ForestGreencheck &  &  &  &  &  &  & 1.28\\ \hline
2021 & \cite{gualtieri2021robotic} & Analytical & \ForestGreencheck &  &  & Sim & Real & 2F & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.26\\ \hline
2021 & \cite{lundell2021ddgc} & Samping & \ForestGreencheck &  &  & Sim & Real & MF & Structured &  &  &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.26\\ \hline
2018 & \cite{gualtieri2018learning} & RL &  &  &  & Sim & Real & 2F & Structured &  & \ForestGreencheck &  &  &  &  &  &  & 1.26\\ \hline
2020 & \cite{Kiatos2020} & Analytical & \ForestGreencheck &  &  & Sim & Real & MF & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.24\\ \hline
2020 & \cite{breyer2021volumetric} & Direct Regression &  &  &  & Sim & Real & 2F & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.23\\ \hline
2016 & \cite{Dexnet1} & Sampling &  &  &  & Sim & Sim & 54 & 43 &  &  &  &  &  &  &  &  & 1.22\\ \hline
\rowcolor[HTML]{ffffff}
2020 & \cite{lu2020multifingered} & Direct Regression &  &  &  & Sim & Real & MF & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.18\\ \hline
2020 & \cite{liu2020deep} & Direct Regression &  &  &  & Sim & Real & MF & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.14\\ \hline
2019 & \cite{ottenhaus2019visuo} & Sampling & \ForestGreencheck &  &  & Sim & Real & MF & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 1.13\\ \hline
2021 & \cite{peng2021selfsupervised} & Sampling &  &  &  & Sim & Real & 2F & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.10\\ \hline
% 2019 & \cite{yan2019dataefficient} & Sampling & \ForestGreencheck &  &  & Sim & Real & 2F & Structured &  & \ForestGreencheck &  &  &  &  & \ForestGreencheck &  & 1.10\\ \hline
2021 & \cite{jiang2021synergies} & Sampling & \ForestGreencheck &  &  & Sim & Real & 2F & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  & \ForestGreencheck &  & 1.08\\ \hline
2020 & \cite{ni2021learning} & Direct Regression &  &  &  & Sim & Real & 2F & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 1.07\\ \hline
2021 & \cite{kasaei2021mvgrasp} & Direct Regression &  &  &  & Real & Real & 2F & \specialcell{Singulated\\Piled} & \ForestGreencheck & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck & \ForestGreencheck &  & 1.04\\ \hline
2020 & \cite{Schaub2020} & Sampling &  &  &  & Real & Real & 2F & Singulated & \ForestGreencheck &  &  &  &  &  &  &  & 1.03\\ \hline
2021 & \cite{Wang2021} & Sampling &  &  &  & Hybrid & Real & 2F & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 1.02\\ \hline
2021 & \cite{wang2021goalauxiliary} & RL &  &  & \ForestGreencheck & Sim & Real & 2F & Singulated &  & \ForestGreencheck &  &  &  & \ForestGreencheck &  &  & 1.02\\ \hline
2018 & \cite{Schmidt2018} & Direct Regression &  &  &  & Sim & Demo & MF & Singulated &  &  &  &  &  &  &  &  & 1.01\\ \hline
2021 & \cite{munoz2021grasping} & Direct Regression &  &  &  & Sim & Demo & 2F & Singulated & \ForestGreencheck & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 1.00\\ \hline
2015 & \cite{bohg2015dataset} & Sampling &  &  &  & Sim & Sim & 3F & Sigulated &  &  &  &  &  &  &  &  & 0.91\\ \hline    
2021 & \cite{Tang2021LearningCP} & RL &  &  &  & Sim & Demo & 2F & Piled &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  &  & 0.82\\ \hline
2020 & \cite{murali2020same} & Sampling &  &  &  & Sim & Demo & 2F & Singulated &  &  &  &  &  &  &  & \ForestGreencheck & 0.64\\ \hline
2016 & \cite{nguyen2016detecting} & Analytical &  & \ForestGreencheck &  & Real & Real & MF & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.64\\ \hline
2018 & \cite{yan2018learning} & Sampling & \ForestGreencheck &  & \ForestGreencheck & Sim & Sim & 2F & Singulated &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 0.59\\ \hline
2017 & \cite{Nguyen2017} & Analytical &  &  &  & Real* & Real & MF & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 0.54\\ \hline
2020 & \cite{Kokic2020} & Direct Regression &  & \ForestGreencheck &  & Sim & Real & MF & Singulated &  &  &  &  &  &  &  & \ForestGreencheck & 0.41\\ \hline
2021 & \cite{Wang_2021_ICCV} & Direct Regression &  &  &  & Hybrid & Real & 2F & Piled &  & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 0.40\\ \hline
2020 & \cite{mandikal2020graff} & RL &  & \ForestGreencheck &  & Sim & Sim & MF & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.37\\ \hline
% 2019 & \cite{tian2019transferring} & 
% Exemplar &  & \ForestGreencheck &  & Sim & Sim & MF & Singulated &  &  &  &  &  & \ForestGreencheck &  &  & 0.36\\ \hline
2020 & \cite{chen2020transferable} & RL &  &  & \ForestGreencheck & Sim & Real & 2F & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 0.34\\ \hline
2020 & \cite{yang2020robotic} & Direct Regression & \ForestGreencheck &  &  & Sim & Sim & 2F & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.33\\ \hline
2017 & \cite{Veres2017} & Sampling &  &  &  & Sim & Sim & MF & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.33\\ \hline
2021 & \cite{wei2021gpr} & Direct Regression &  &  &  & Sim & Real & 2F & Piled &  & \ForestGreencheck & \ForestGreencheck & \ForestGreencheck &  &  &  &  & 0.32\\ \hline
2019 & \cite{Ardon2019} & Direct Regression &  & \ForestGreencheck &  & Sim & Real & 2F & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.28\\ \hline
% % 2020 & \cite{Riccardo2020} & GPD &  & \ForestGreencheck &  & - & - &  &  &  &  &  &  &  &  &  &  & 0.26\\ \hline
2021 & \cite{li2021simultaneous} & Direct Regression &  & \ForestGreencheck &  & Sim & Real & 2F & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  &  &  & \ForestGreencheck & 0.19\\ \hline
2021 & \cite{corsaro2021learning} & Sampling &  &  &  & Sim & Real & MF & Structured &  & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 0.19\\ \hline
2020 & \cite{patten2020dgcm} & Exemplar &  &  &  & Sim & Real & 2F & Singulated &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 0.18\\ \hline
2020 & \cite{li2020learning} & Analytical &  & \ForestGreencheck &  & Sim & Sim & 2F & Singulated &  & \ForestGreencheck &  &  &  &  & \ForestGreencheck &  & 0.13\\ \hline
2020 & \cite{jeng2020gdn} & Direct Regression &  &  &  & Sim & Sim & 2F & \specialcell{Singulated\\Structured} &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck & 0.09\\ \hline
2018 & \cite{Torii2018} & Analytical & \ForestGreencheck &  &  & Sim & Sim & 3F & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.09\\ \hline
2017 & \cite{zhou20176dof} & Sampling &  &  &  & Sim & Sim & 3F & Singulated &  &  &  &  & \ForestGreencheck &  &  &  & 0.08\\ \hline
2019 & \cite{Goncalves2019} & Sampling &  &  &  & Sim & Real & 3F & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.07\\ \hline
2021 & \cite{Cortes2021} & Direct Regression &  &  & \ForestGreencheck & Real & Real & MF & Structured &  & \ForestGreencheck &  &  &  &  &  &  & 0.06\\ \hline
2019 & \cite{aktas2019deep} & Sampling &  &  & \ForestGreencheck & Sim & Real & MF & Singulated &  & \ForestGreencheck &  &  & \ForestGreencheck &  &  &  & 0.03\\ \hline
2020 & \cite{Riedlinger2020} & Sampling &  &  &  & Sim & Sim & 2F & Singulated &  &  &  &  &  &  &  & \ForestGreencheck & 0.03\\ \hline
2020 & \cite{avigal20206dof} & Shape Completion & \ForestGreencheck &  &  & Sim & Sim & 2F & Singulated & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  &  & 0.02\\ \hline
2020 & \cite{Wang2020} & Direct Regression &  &  &  & Sim & Real & MF/2F & \specialcell{Structured\\Piled} &  & \ForestGreencheck &  &  &  &  &  &  & 0.01\\ \hline
2021 & \cite{Ren2021} & Sampling &  &  &  & Sim & Real & 2F & Structured &  & \ForestGreencheck &  & \ForestGreencheck &  & \ForestGreencheck &  &  & 0.01\\ \hline
2021 & \cite{Li2021} & Direct Regression &  &  &  & Sim & Real & MF & Singulated &  & \ForestGreencheck &  &  &  &  &  &  & 0.01\\ \hline
2021 & \cite{kawakami2021learning} & RL &  &  & \ForestGreencheck & Sim & Sim & 2F & Singulated &  &  &  &  &  &  &  &  & 0.00\\ \hline
2021 & \cite{wencatgrasp} & Sampling &  & \ForestGreencheck &  & Sim & Real & 2F & Piled &  & \ForestGreencheck &  &  &  &  &  &  & 0.00\\ \hline
2021 & \cite{Schuab2021} & Sampling & \ForestGreencheck &  &  &  & Real & 2F & Singulated & \ForestGreencheck & \ForestGreencheck &  &  &  &  &  &  & 0.00\\ \hline
2021 & \cite{chavandafle2021object} & Analytical & \ForestGreencheck &  &  & Sim & Real & 2F & Structured &  & \ForestGreencheck &  &  &  &  &  & \ForestGreencheck & 0.00\\ \hline



\caption{The papers included in this systematic review ordered by our impact score (Section~\ref{sec:method}).
The various properties are presented for easy comparison.
``PD" indicates whether the grasping approach was partial 6-DoF. ``MF" represents a Multi-Fingered hand, while ``2F", ``3F" refer to Two-Finger and Three Finger respectively.
``SC" referes to if the appraoch used Shape Completion. ``SA" refers to Semantics/Affordances.
``SR", ``Cov", ``Com", ``CT", ``IOU" and ``P" refer to Success Rate, Coverage Rate, Completion Rate, Computation Time, Intersection of Union and Precision which were the metrics used in the paper, refer to Sec.~\ref{sec:metrics}.
``Impact" is the impact described in Section~\ref{quality_score}. *This data contains no grasping information.\\}
\label{big_table}
\end{longtable}
